LSA-T: The first continuous Argentinian Sign Language dataset for Sign Language Translation

Sign language translation (SLT) is an active field of study that encompasses human-computer interaction, computer vision, natural language processing and machine learning. Progress on this field could lead to higher levels of integration of deaf people. This paper presents, to the best of our knowledge, the first continuous Argentinian Sign Language (LSA) dataset. It contains 14,880 sentence level videos of LSA extracted from the CN Sordos YouTube channel with labels and keypoints annotations for each signer. We also present a method for inferring the active signer, a detailed analysis of the characteristics of the dataset, a visualization tool to explore the dataset and a neural SLT model to serve as baseline for future experiments.

==> Comentarios_AleR.tex <==
A discutir -------------------------------------------------
- Si no crees que tenga algùn valor el experimenrto con la RN creo que es mejor no poner eso .. porque no tiene sentido hacer un experimento que se supone que no funcione, y se muestra que no funciona, porque eso n aporta conocimiento ... casi eso es lo que saldrìa de la frase " Then it is not surprising that given the complexity
of the presented dataset the models did not obtained good results" ... en mi opinion, enfocar el trabajo al dataset, poniendo màs informaciòn sobre èl, podrìa quedar mejor que asi, porque la parte de RN creo que le bajara puntos .. a menos que haya algo interesante que mostrar de los resultados

- En el resumen creo que hay que resaltar lo que significa que sea "continuo" porque eso es lo que da el matiz novedoso.
- En la seccion 2 creo que conviene separar en lo posible lo otro existente (lo previo) del tuyo, quizas indicando luego de exponer lo previo la necesidad del tuyo, y ahi decir sus singularidades, reforzado con la tabla.

- hablas de "trigrams" aqui y no es una base de datos en que el texto sea la informacion primaria... si es relevante, creo que merece explicarlo porque creo que queda claro la utilidad de eso aqui

- Entiendo la necesidad de la nueva metrica, pero seguro los revisores exigiran una mayor justificacion y el problema de las otras mètricas ... incluso, creo que debes dejar claro si considerar que las comparaciones con este baseline que das siempre debe hacerse respecto a esta nueva metrica, o habrìa otra que tendria sentido para la comparacion


A RESOLVER ------------------------------------------

- En la primera linea de 1.1 tratar de evitar que quede dividido "LSA-T"
https://tex.stackexchange.com/questions/182569/how-to-manually-set-where-a-word-is-split

- EN la tabla. Queda Raro FHD.  Se solucionaría si ponemos Language= Argentinian ?

==> other/playlists.tex <==
Videos were taken from four playlists:

\begin{itemize}
    
    \item "Resumen semanal" (\textit{Weekly summary}) is the main playlist from where the videos were taken. Its videos follow the format described above where two hosts present the news from the latest weeks. It features varied topics, interviews, and special sections like movies or horoscopes.
    
    \item "Ley federal LSA" (\textit{LSA Federal Law}) presents in a similar format as "Resumen semanal" news about a law project about LSA in Argentina.
    
    \item "Último momento" (\textit{Breaking News}) has videos from people in different places presenting breaking news. Videos from this playlist usually have lower quality than the other playlists and were not recorded in such a professional way. They also cover a big variety of topics (no video presents the same piece of news as other). Therefore, this playlist is considered particularly difficult for a model to learn.
    
    \item "CN Sordos ecología" (\textit{CN sordos ecology}) is a section where only one presenter talks about topics regarding ecology. Videos from this playlist were not recorded in a studio like the ones from "Resumen Semanal", but have better quality than those in "Último momento".
    
\end{itemize}

Figure \ref{fig:channel_screenshots} shows screenshots of the mentioned playlists. The different peculiarities of each one were taken into account to build different test, train, and validation sets, some expected to be more or less difficult for a model to learn depending on which playlist the videos were taken from. How this was done is described in section \ref{subsec:train_test_split}.

The videos were taken from the aforementioned playlists, but mainly from "Resumen semanal" as it was the larger playlist and subtitles were available for most of its videos. Figure \ref{fig:hist_videos_by_playlists} shows the amount of videos taken from each playlist.

\input{figures/videos_by_playlists}


==> other/videos_by_playlists.tex <==
\begin{figure}
    \includegraphics[width=\textwidth]{images/hist_videos_by_playlists.png}
    \caption{Amount of clips taken from each playlist.} \label{fig:hist_videos_by_playlists}
\end{figure}
